Large-scale weakly-supervised pre-training for video action recognition

Current fully-supervised video datasets consist of only a few hundred thousand videos and fewer than a thousand domain-specific labels. This hinders the progress towards advanced video architectures. This paper presents an in-depth study of using large volumes of web videos for pre-training video models for the task of action recognition. Our primary empirical finding is that pre-training at a very large scale (over 65 million videos), despite on noisy social-media videos and hashtags, substantially improves the state-of-the-art on three challenging public action recognition datasets. Further, we examine three questions in the construction of weakly-supervised video action datasets. First, given that actions involve interactions with objects, how should one construct a verb-object pre-training label space to benefit transfer learning the most? Second, frame-based models perform quite well on action recognition; is pre-training for good image features sufficient or is pre-training for spatio-temporal features valuable for optimal transfer learning? Finally, actions are generally less well-localized in long videos vs. short videos; since action labels are provided at a video level, how should one choose video clips for best performance, given some fixed budget of number or minutes of videos?

==> abstract_matt.tex <==
Current fully-supervised video datasets consist of only a few hundred thousand videos and fewer than a thousand domain-specific labels due to high annotation costs. This lack of large-scale datasets has slowed progress towards advanced video architectures. This work presents an in-depth study of the role of large volumes of web videos for pre-training video models for action recognition. Our primary empirical finding is that pre-training at a very large scale (over $65$ million videos and $10,000$ action labels), despite on noisy social-media videos and hashtags, substantially improves the state-of-the-art on four challenging public action recognition datasets. Further, we examine three questions in the construction of weakly-supervised video action datasets.  First, actions take objects, so how should one construct the best \emph{verb-object} label space for transfer learning?  Second, frame-based models perform quite well on action recognition; is pre-training for good image features sufficient for optimal transfer learning, or is pre-training spatio-temporal features valuable?  Finally, actions are generally less well-localized in long videos vs short videos; labels are given at video level, how should we choose video clips for best performance, given some fixed budget of videos or compute?



==> intro.tex <==
\section{Introduction}
Pre-training on large datasets followed by fine-tuning on target tasks is an established practice \cite{decaf, imagenetTransfer} as it yields strong performance benefits especially when the target datasets are small \cite{segment, poseEstimation, oflow, posetrack, r2plus1D, nonlocal}. Given the well-known challenges in constructing large-scale fully-supervised video datasets, it is intuitive that large-scale pre-training is even more vital for video tasks. 

Recent studies \cite{uruImage, jft, laurens} have clearly demonstrated that pre-training on hundreds of millions (billions) of noisy web images significantly boosts the state-of-the-art in object classification. While web images primarily tackle \textit{label noise} (i.e., missing or incorrect object labels), videos in the wild additionally face \textit{temporal noise} due to the lack of localization of action labels. Specifically, real-world videos predominantly involve composite actions, with each action occupying only a very small fraction of the sequence. Thus, it is not immediately apparent if the successes from the image domain \cite{uruImage, jft, laurens} should trivially translate to video models \cite{r2plus1D, 3d1, 3d2, 3d3, nonlocal} at all. Towards this end, we address several unexplored questions related to large-scale pre-training using web videos for action recognition. 

However, using web videos and the associated noisy metadata such as hashtags during pre-training poses crucial challenges regarding the design of an appropriate pre-training label space. For example, while image task labels are restricted to scenes and objects (i.e., nouns), action labels (eg: \textit{catching a fish}) are more complex and typically involve one (or more) objects and verbs to capture their interactions. Given this, should the pre-training label space be noun-focused (\textit{\#fish}) or  verb-focused (\textit{\#catch}) or an appropriate combination of both (\textit{\#catchingfish}), or target task-focused altogether? How many such labels are sufficient for effective pre-training and how diverse should they be? 

In addition to understanding the pre-training label space characteristics, the temporal dimension itself opens doors for several interesting questions. Given the massive amounts of web videos available, what videos should one choose from for pre-training? How does pre-training on longer videos which lack temporally-localized actions compare with pre-training on short videos that presumably have better localization? At a more fundamental level, should we even pre-train on video clips at all given the development of strategies such as inflation\cite{i3d} to exclusively transfer the benefits from image pre-training to video models?
%We perform an in-depth analysis of large scale (tens of millions of videos), weakly-supervised pre-training with videos in-the-wild. 

In this work, we address all these questions in great detail. Our key aim is to improve the learned video feature representations by focusing exclusively on the complementary direction of training data instead of model-architecture design. Specifically, we leverage over $65$ million public, user-generated videos from a social media website and use the associated hashtags as labels for pre-training. The label noise and temporal noise makes our training framework \textit{weakly-supervised}. Unlike \underline{all} existing fully-supervised video datasets \cite{thumos, hmdb, kth, hollywood, ucf, kinetics, soa, momentsintime} which involved expensive annotation requirements, our training data is truly extensible to billion-scale without incurring any annotation costs. We effectively tackle the aforementioned complexities related to label space and various temporal aspects, and demonstrate significant performance gains on various target tasks. Overall, we summarize our findings:
\begin{packed_enum}
% \vspace{-0.05in}
\item {\textbf{Large-scale weak-supervision is extremely beneficial:}} We show that for videos, large-scale data, despite not providing strong supervision, tremendously helps models of varied capacities in learning better features. Our experiments clearly demonstrate that content diversity and scale outdo label and temporal noise. 
\item \textbf{Impact of data volume and model capacity:} We report interesting findings on the effect of pre-training data size, data sampling strategies, and model capacities. For instance, similar to the previous studies on images \cite{uruImage}, we find that increasing the model capacity (Sec. \ref{sec:capacity}) improves the performance, however, unlike in images \cite{uruImage}, increasing the number of training videos beyond $10-20$ million videos does not boost performance (Sec. \ref{sec:datapoints}).
%\item \textbf{Pre-training label design is crucial:} 
\item \textbf{What is a suitable pre-training video label space?}
Using hashtags, we systematically construct pre-training label sets that vary in their cardinality and type, i.e., verbs, nouns, target task labels, and exhaustive combinations of verbs and nouns, and study their effect target tasks (Sec. \ref{sec:labelEffect}). One key finding is that as in \cite{uruImage}, pre-training labels that match the target tasks improve performance.
\item \textbf{Do we need pre-training on video data?} 
We investigate the true value of pre-training using video data and show that it is necessary to use videos as opposed to video frames or images followed by inflation~\cite{i3d} to achieve better performance when operating at scale (Sec. \ref{sec:image2video}). 
\item \textbf{Short vs. long videos for pre-training?} We study the effect of pre-training on shorter and longer duration videos (Sec. \ref{sec:vidLengths}) and show that (a) for a given pre-training video length budget, it is beneficial to choose a large number of short videos as they supply succinct localized actions compared to fewer number of long videos, (b) for a given pre-training number of videos budget, choosing longer videos is beneficial as they offer diverse content. 
\item {\textbf{State-of-the-art results:}} We achieve a top-1 video accuracy of $\boldsymbol{80.49\%}$ on Kinetics, a $2.8\%$ boost over the previous state-of-the-art \cite{nonlocal} (Sec. \ref{sec:sota}). While the performance gains in \cite{nonlocal} were achieved via architectural innovation, increased compute, etc., our performance boost is purely from pre-training a simple architecture (R(2+1)D \cite{r2plus1D}) at scale. On Epic Kitchens action recognition challenge \cite{epicKitchens}, we achieve an mAP of $\boldsymbol{24.9\%}$ on unseen verb-noun pairs, an improvement of $\sim 8.5\%$ over the top entry in the leadership board at the time of  submission. 
\end{packed_enum}
%We do a careful in-depth analysis of various temporal aspects of videos. 
%On the other hand, while scaling to billions of images showed significant gains \cite{jft, uruImage}, we did not observe such boosts after about $10$ million pre-training videos.  
%\matt{At his point a natural question is how many distinct frames the image and video models each saw, and then there's a question of diversity of visual information which maybe we can't answer but should recognize.  I.e. are we actually exhausting the visual diversity in our label space?  It'll be easier to talk to this when some of the more recent experiments are done.}
%\note{@Matt: We are actually seeing improvement with more data. Do you still think there is value in comparing 3.5B images with the video model processing 492.5M videos in total of 32-frame input?}
%Given the well-known challenges in constructing large-scale fully-supervised video datasets, 
%what videos should one choose for pre-training from potentially billions of public web videos? Given a fixed training budget, should we choose - short videos having presumably good temporal localization of actions or longer videos which supply correlated side information and hence more content diversity?  
%Given fixed pre-training hours of video, should we choose a large number of short duration videos for pre-training or a smaller number of long videos. 
%We address this question in ths work and train video models on millions of videos using weak-supervision
%Similar to these, our approach also suffers from limited information, since hashtags mostly reflect objects 174 (nouns) and may not provide action-related information 175 contained in the video
%The effect of this temporal noise in web videos on the state-of-the-art video models \cite{r2plus1D, 3d1, 3d2, 3d3, nonlocal} when pre-trained at very large-scale is not immediately unclear. 
%\matt{Call out temporal localization here -- also mention that images are, by design, well localized 'good' frames, or people wouldn't post them, which is rather unlike a typical frame of video} 
%While all weakly-supervised datasets \cite{uruImage, jft, laurens} suffer from noisy, missing, or incorrect labels -- all due to lack of clear annotation supervision -- videos \textit{in-the-wild} face an additional challenge of the lack of \textit{temporal localization} of action labels. Specifically, real-world videos predominantly involve different composite actions with each action occupying only a very small fraction of the sequence. The extent of influence of this temporal noise on the state-of-the-art video models \cite{r2plus1D, 3d1, 3d2, 3d3, nonlocal} is not immediately unclear. 
%are available in abundance and therefore provide an opportunity as well as a challenge of choosing the right subset of them for training.
%Video action label space is fundamentally different from image tasks thus posing further challenges in terms of designing the right pre-training label space.

==> intro_deepti.tex <==
\section{Introduction}
Pre-training on large datasets followed by fine-tuning on target tasks is an established practice \cite{decaf, imagenetTransfer} as it yields strong performance benefits especially when the target datasets are small \cite{segment, poseEstimation, oflow, posetrack, r2plus1D, nonlocal}. Current fully-supervised video datasets consist of only a few hundred thousand videos and less than a thousand domain-specific labels due to high annotation costs. Hence, it is intuitive that weakly-supervised pre-training at scale is even more vital for video tasks. Recent studies \cite{uruImage, jft, laurens} have clearly demonstrated that pre-training on hundreds of millions (billions) of noisy web images with weak supervision significantly boost the state-of-the-art in object classification. However, aside from the ill-posed nature of action labels vocabulary, videos introduce an additional dimension of time (hence motion). Also, while social-media images are, by design, well-localized with regards to the associated labels, the same is not often true for videos.
%\matt{Call out temporal localization here -- also mention that images are, by design, well localized 'good' frames, or people wouldn't post them, which is rather unlike a typical frame of video} 
Thus, it is not immediately apparent if the successes from the image domain \cite{uruImage, jft, laurens} should trivially translate to videos at all.

While all weakly-supervised datasets \cite{uruImage, jft, laurens} suffer from noisy, missing, or incorrect labels -- all due to lack of clear annotation supervision -- videos \textit{in-the-wild} face an additional challenge of the lack of \textit{temporal localization} of action labels. Specifically, real-world videos predominantly involve different composite actions with each action occupying only a very small fraction of the sequence. The extent of influence of this temporal noise on the state-of-the-art video models \cite{r2plus1D, 3d1, 3d2, 3d3, nonlocal} is not immediately unclear. 

Going beyond this, large-scale weakly-supervised video pre-training poses several interesting questions and challenges. Web videos along with the associated noisy metadata are available in abundance and therefore provide an opportunity as well as a challenge of choosing the right subset of them for training. As an example, action labels (\textit{catching a fish}) typically involve one (or more) objects and verbs to capture their interactions and hence are more complex. Should training be done with only objects (\textit{\#fish}) or scenes-specific hashtags as is typically the case with image tasks, or, should the verbs (\textit{\#catch}) be given more importance, or, perhaps select an appropriate combination of noun and verbs hashtags (\textit{\#catchingfish})? How many hashtags are enough for video training and how diverse should they be? \note{We need a good way to introduce the usage of hashtags}

In addition to understanding the characteristics of the pre-training label space, the temporal dimension opens doors for several interesting questions. For instance, what videos should one choose for pre-training from potentially billions of public web videos? Given a fixed training budget, should we choose - short videos having presumably good temporal localization of actions or longer videos which supply correlated side information and hence more content diversity?  Given fixed pre-training hours of video, should we choose a large number of short duration videos for pre-training or a smaller number of long videos. Finally, a strategy such as inflation\cite{i3d} has been specifically proposed to leverage image pre-training to bootstrap video models. Given this and the established leaping benefits from pre-training on billions of images \cite{uruImage}, should we pre-train on video clips at all?

In this work, we address all the above questions. We perform an in-depth analysis of large scale (tens of millions of videos), weakly-supervised pre-training with videos in-the-wild. Our aim is to improve the learned video feature representations by focusing exclusively on the complementary direction of training data instead of model-architecture design. Specifically, we leverage over $65$ million public, user-generated videos from a social media website and use the associated hashtags as labels for pre-training. Unlike \underline{all} existing fully-supervised video datasets \cite{thumos, hmdb, kth, hollywood, ucf, kinetics, soa, momentsintime} which involved expensive annotation requirements, our training data is truly extensible to billion-scale without incurring any annotation costs. Despite the aforementioned complexities, we empirically observe that video models, like images, hugely benefit from this large-scale pre-training approach.
Overall, we summarize our contributions:
\begin{packed_enum}
\vspace{-0.1in}
\item We show that for videos, large-scale data, despite not providing strong supervision, tremendously helps models of varied capacities in learning better features.Our best model achieves a top-1 video accuracy of $\boldsymbol{80.49\%}$ on Kinetics which is a $2.8\%$ boost over the previous state-of-the-art \cite{nonlocal} (Sec. \ref{sec:sota}).While the performance gains in \cite{nonlocal} were achieved via architectural innovation, increased compute, etc. our performance boost is purely from pre-training a simple architecture (R(2+1)D \cite{r2plus1D} on very large-scale dataset. On Epic Kitchens action recognition challenge \cite{epicKitchens}, we achieve an mAP of $\boldsymbol{24.9\%}$ on unseen verb-noun pairs, an improvement of around $8.5\%$ over the top entry in the leadership board at the time of the submission of this manuscript. Thus, our experiments clearly demonstrate that content diversity and scale outdo label and data noise.
\item We perform a series of ablation studies, such as the effect of pre-training data size, model capacity, etc., and make several interesting observations. For instance, similar to previous studies on images \cite{uruImage}, we find that increasing the model capacity (Sec. \ref{sec:capacity}) improves the performance on target tasks. However, unlike in \cite{jft, uruImage}, increasing the number of training videos (Sec. \ref{sec:datapoints}) does not boost performance after $10-20$ million videos for Kinetics and Epic-Kitchens. 
\item We find that as in \cite{uruImage}, constructing pre-training label sets that match the target tasks yields improved performance. While the labels that combine verb and noun intuitively should provide better supervision than using nouns or verbs independently, we observe that they actually perform worse due to long tail distribution. \note{Dhruv - this long tailed distribution of verb+noun is not very clear. Perhaps should not be mentioned here.}
%On the other hand, while scaling to billions of images showed significant gains \cite{jft, uruImage}, we did not observe such boosts after about $10$ million pre-training videos.  
%\matt{At his point a natural question is how many distinct frames the image and video models each saw, and then there's a question of diversity of visual information which maybe we can't answer but should recognize.  I.e. are we actually exhausting the visual diversity in our label space?  It'll be easier to talk to this when some of the more recent experiments are done.}
%\note{@Matt: We are actually seeing improvement with more data. Do you still think there is value in comparing 3.5B images with the video model processing 492.5M videos in total of 32-frame input?}
\item We do a careful in-depth analysis of various temporal aspects of videos. We investigate the true value of pre-training using video data and show that it is necessary to pre-train using videos as opposed to video frames or images followed by inflation~\cite{i3d} to achieve better performance when operating at scale (Sec. \ref{sec:image2video}). We also study the effect of pre-training on shorter and longer duration videos to understand the effect of temporal noise and diversity (Sec. \ref{sec:vidLengths}) and show that longer videos supply more content diversity while short videos supply succinct localized actions, both leading to better pre-trained models. 
\end{packed_enum}

%Given the well-known challenges in constructing large-scale fully-supervised video datasets, 

==> intro_matt.tex <==
\section{Introduction}
It is well-established \cite{decaf, imagenetTransfer} that pre-training on large datasets followed by fine-tuning on target tasks boosts performance, especially when the target datasets are small \cite{segment, poseEstimation, oflow, posetrack, r2plus1D, nonlocal}. 
Given the well-known complexities and expense in constructing large-scale fully-supervised video datasets, it is intuitive that large-scale weakly-supervised pre-training is even more vital for video tasks than for images. 

Recent studies \cite{uruImage, jft, laurens} have clearly demonstrated that pre-training on hundreds of millions (billions) of noisy web images significantly boosts the state-of-the-art in object classification. While one would certainly hope that successes would carry over from images \cite{uruImage, jft, laurens} to video \cite{r2plus1D, 3d1, 3d2, 3d3, nonlocal}, action recognition in video has some features which make this less obvious than it might appear and also presents challenges in dataset construction which are absent from the image domain.

First, while web images primarily tackle \textit{label noise} (i.e., missing or incorrect object labels), videos in the wild additionally face \textit{temporal noise} due to lack of localization of action labels.  In real-world videos, any given action typically occupies only a very small fraction of the sequence.  In stark contrast, a typical web image is a particular moment in time, carefully selected by its creator for maximal relevance, salience, and so on.

Second, in prior work on images, labels were restricted to scenes and objects (i.e., nouns).  However, action labels (eg: \textit{catching a fish}) are more complex, typically involving at least one verb-object pair.  Further, even at large scale, many valid verb-object pairs may be observed rarely or never at all; for example, "catching a bagel" is an entirely plausible action, but rarely observed.  Is it more effective to pre-train on labels chosen from marginal distributions of nouns and verbs, do we need to pre-train on the incomplete but observed portion of the joint distribution of (verb, noun) labels, or do we need to focus entirely on the target task's labels? How many such labels are sufficient for effective pre-training and how diverse should they be? 

Third, the temporal dimension raises several interesting questions. By analogy to images, short videos should be better-localized than longer videos; we both investigate this assumption and also ask how weaker localization affects pre-training.  Longer videos contain more frames, but short videos presumably contain more relevant frames; what is the best choice of video lengths when constructing a pre-training dataset? We consider this for a fixed number of minutes of video, and separately for a fixed compute budget, and arrive at different answers in each case.

Finally, we question whether pre-training on video (vs images) is even necessary.  Both frame-based models and image-based pre-training methods like inflation \cite{i3d} have been successful in action recognition. Is pre-training on video clips actually worth the increased compute required?  Or are strong 2D features sufficient, and temporal features like motion comparatively simple and easy to learn in our current models?


In this work, we address all these questions in great detail. Our key aim is to improve the learned video feature representations by focusing exclusively on the complementary direction of training data instead of model-architecture design. Specifically, we leverage over $65$ million public, user-generated videos from a social media website and use the associated hashtags as labels for pre-training. The label noise and temporal noise makes our training framework \textit{weakly-supervised}. Unlike \underline{all} existing fully-supervised video datasets \cite{thumos, hmdb, kth, hollywood, ucf, kinetics, soa, momentsintime} which involved expensive annotation requirements, our training data is truly extensible to billion-scale without incurring any annotation costs. We effectively tackle the aforementioned complexities related to label space and various temporal aspects, and demonstrate significant performance gains on various target tasks. Overall, we summarize our findings:
\begin{packed_enum}
% \vspace{-0.05in}
\item {\textbf{Large-scale weak-supervision is extremely beneficial:}} We show that for videos, large-scale data, despite not providing strong supervision, tremendously helps models of varied capacities in learning better features. Our experiments clearly demonstrate that content diversity and scale outdo label and temporal noise. 
\item \textbf{Impact of data volume and model capacity:} We report interesting findings on the effect of pre-training data size, data sampling strategies, and model capacities. For instance, similar to the previous studies on images \cite{uruImage}, we find that increasing the model capacity (Sec. \ref{sec:capacity}) improves the performance, however, unlike in images \cite{uruImage}, increasing the number of training videos beyond $10-20$ million videos does not boost performance (Sec. \ref{sec:datapoints}).
%\item \textbf{Pre-training label design is crucial:} 
\item \textbf{What is a suitable pre-training video label space?}
Using hashtags, we systematically construct pre-training label sets that vary in their cardinality and type, i.e., verbs, nouns, target task labels, and exhaustive combinations of verbs and nouns, and study their effect target tasks (Sec. \ref{sec:labelEffect}). One key finding is that as in \cite{uruImage}, pre-training labels that match the target tasks improve performance.
\item \textbf{Do we need pre-training on video data?} 
We investigate the true value of pre-training using video data and show that it is necessary to use videos as opposed to video frames or images followed by inflation~\cite{i3d} to achieve better performance when operating at scale (Sec. \ref{sec:image2video}). 
\item \textbf{Short vs. long videos for pre-training?} We study the effect of pre-training on shorter and longer duration videos (Sec. \ref{sec:vidLengths}) and show that (a) for a given pre-training video length budget, it is beneficial to choose a large number of short videos as they supply succinct localized actions compared to fewer number of long videos, (b) for a given pre-training number of videos budget, choosing longer videos is beneficial as they offer diverse content. 
\item {\textbf{State-of-the-art results:}} We achieve a top-1 video accuracy of $\boldsymbol{80.49\%}$ on Kinetics, a $2.8\%$ boost over the previous state-of-the-art \cite{nonlocal} (Sec. \ref{sec:sota}). While the performance gains in \cite{nonlocal} were achieved via architectural innovation, increased compute, etc., our performance boost is purely from pre-training a simple architecture (R(2+1)D \cite{r2plus1D}) at scale. On Epic Kitchens action recognition challenge \cite{epicKitchens}, we achieve an mAP of $\boldsymbol{24.9\%}$ on unseen verb-noun pairs, an improvement of $\sim 8.5\%$ over the top entry in the leadership board at the time of  submission. 
\end{packed_enum}
%We do a careful in-depth analysis of various temporal aspects of videos. 
%On the other hand, while scaling to billions of images showed significant gains \cite{jft, uruImage}, we did not observe such boosts after about $10$ million pre-training videos.  
%\matt{At his point a natural question is how many distinct frames the image and video models each saw, and then there's a question of diversity of visual information which maybe we can't answer but should recognize.  I.e. are we actually exhausting the visual diversity in our label space?  It'll be easier to talk to this when some of the more recent experiments are done.}
%\note{@Matt: We are actually seeing improvement with more data. Do you still think there is value in comparing 3.5B images with the video model processing 492.5M videos in total of 32-frame input?}
%Given the well-known challenges in constructing large-scale fully-supervised video datasets, 
%what videos should one choose for pre-training from potentially billions of public web videos? Given a fixed training budget, should we choose - short videos having presumably good temporal localization of actions or longer videos which supply correlated side information and hence more content diversity?  
%Given fixed pre-training hours of video, should we choose a large number of short duration videos for pre-training or a smaller number of long videos. 
%We address this question in ths work and train video models on millions of videos using weak-supervision
%Similar to these, our approach also suffers from limited information, since hashtags mostly reflect objects 174 (nouns) and may not provide action-related information 175 contained in the video
%The effect of this temporal noise in web videos on the state-of-the-art video models \cite{r2plus1D, 3d1, 3d2, 3d3, nonlocal} when pre-trained at very large-scale is not immediately unclear. 
%\matt{Call out temporal localization here -- also mention that images are, by design, well localized 'good' frames, or people wouldn't post them, which is rather unlike a typical frame of video} 
%While all weakly-supervised datasets \cite{uruImage, jft, laurens} suffer from noisy, missing, or incorrect labels -- all due to lack of clear annotation supervision -- videos \textit{in-the-wild} face an additional challenge of the lack of \textit{temporal localization} of action labels. Specifically, real-world videos predominantly involve different composite actions with each action occupying only a very small fraction of the sequence. The extent of influence of this temporal noise on the state-of-the-art video models \cite{r2plus1D, 3d1, 3d2, 3d3, nonlocal} is not immediately unclear. 
%are available in abundance and therefore provide an opportunity as well as a challenge of choosing the right subset of them for training.
%Video action label space is fundamentally different from image tasks thus posing further challenges in terms of designing the right pre-training label space.

==> intro_nov13_dg.tex <==
\section{Introduction}
Pre-training on large datasets followed by fine-tuning on target tasks is an established practice \cite{decaf, imagenetTransfer} as it yields strong performance benefits especially when the target datasets are small \cite{segment, poseEstimation, oflow, posetrack, r2plus1D, nonlocal}. Current fully-supervised video datasets consist of only a few hundred thousand videos and less than a thousand domain-specific labels due to high annotation costs. Hence, it is intuitive that large-scale pre-training is even more vital for video tasks. 

Recent studies \cite{uruImage, jft, laurens} have clearly demonstrated that pre-training on hundreds of millions (billions) of noisy web images significantly boosts the state-of-the-art in object classification. While web images primarily tackle \textit{label noise} (i.e., missing or incorrect object labels), videos in the wild additionally face \textit{temporal noise} due to the lack of localization of action labels. Specifically, real-world videos predominantly involve composite actions, with each action occupying only a very small fraction of the sequence. Thus, it is not immediately apparent if the successes from the image domain \cite{uruImage, jft, laurens} should trivially translate to video models \cite{r2plus1D, 3d1, 3d2, 3d3, nonlocal} at all. Towards this end, we address several unexplored questions related to large-scale pre-training using web videos for action recognition. 

However, using web videos and the associated noisy metadata such as hashtags during pre-training poses crucial challenges regarding the design of an appropriate pre-training label space. For example, while image task labels are restricted to scenes and objects (i.e., nouns), action labels (eg: \textit{catching a fish}) are more complex and typically involve one (or more) objects and verbs to capture their interactions. Given this, should the pre-training label space be noun-focused (\textit{\#fish}) or  verb-focused (\textit{\#catch}) or an appropriate combination of both (\textit{\#catchingfish}), or target task-focused altogether? How many such labels are sufficient for effective pre-training and how diverse should they be? 

In addition to understanding the pre-training label space characteristics, the temporal dimension itself opens doors for several interesting questions. Given the massive amounts of web videos available, what videos should one choose from for pre-training? How does pre-training on longer videos which lack temporally-localized actions compare with pre-training on short videos that presumably have better localization? At a more fundamental level, should we even pre-train on video clips at all given the development of strategies such as inflation\cite{i3d} to exclusively transfer the benefits from image pre-training to video models?
%We perform an in-depth analysis of large scale (tens of millions of videos), weakly-supervised pre-training with videos in-the-wild. 

In this work, we address all these questions in great detail. Our key aim is to improve the learned video feature representations by focusing exclusively on the complementary direction of training data instead of model-architecture design. Specifically, we leverage over $65$ million public, user-generated videos from a social media website and use the associated hashtags as labels for pre-training. The label noise and temporal noise makes our training framework \textit{weakly-supervised}. Unlike \underline{all} existing fully-supervised video datasets \cite{thumos, hmdb, kth, hollywood, ucf, kinetics, soa, momentsintime} which involved expensive annotation requirements, our training data is truly extensible to billion-scale without incurring any annotation costs. We effectively tackle the aforementioned complexities related to label space and various temporal aspects, and demonstrate significant performance gains on various target tasks. Overall, we summarize our findings:
\begin{packed_enum}
\vspace{-0.04in}
\item {\textbf{Large-scale weak-supervision is extremely beneficial:}} We show that for videos, large-scale data, despite not providing strong supervision, tremendously helps models of varied capacities in learning better features. Our experiments clearly demonstrate that content diversity and scale outdo label and temporal noise. 
\item \textbf{Impact of data volume and model capacity:} We report interesting findings on the effect of pre-training data size, data sampling strategies, and model capacities. For instance, similar to the previous studies on images \cite{uruImage}, we find that increasing the model capacity (Sec. \ref{sec:capacity}) improves the performance, however, unlike in images \cite{uruImage}, increasing the number of training videos beyond $10-20$ million videos does not boost performance (Sec. \ref{sec:datapoints}).
%\item \textbf{Pre-training label design is crucial:} 
\item \textbf{What is a suitable pre-training video label space?}
Using hashtags, we systematically construct pre-training label sets that vary in their cardinality and type, i.e., verbs, nouns, target task labels, and exhaustive combinations of verbs and nouns, and study their effect target tasks (Sec. \ref{sec:labelEffect}). One key finding is that as in \cite{uruImage}, pre-training labels that match the target tasks improve performance.
\item \textbf{Do we need pre-training on video data?} 
We investigate the true value of pre-training using video data and show that it is necessary to use videos as opposed to video frames or images followed by inflation~\cite{i3d} to achieve better performance when operating at scale (Sec. \ref{sec:image2video}). 
\item \textbf{Short vs. long videos for pre-training?} We study the effect of pre-training on shorter and longer duration videos in great detail (Sec. \ref{sec:vidLengths}) and show that (a) for a given pre-training video length budget, it is beneficial to choose a large number of short videos as they supply succinct localized actions compared to fewer number of long videos, (b) for a given pre-training number of videos budget, choosing longer videos is beneficial as they offer diverse content. 
\item {\textbf{State-of-the-art results:}} We achieve a top-1 video accuracy of $\boldsymbol{80.49\%}$ on Kinetics, a $2.8\%$ boost over the previous state-of-the-art \cite{nonlocal} (Sec. \ref{sec:sota}). While the performance gains in \cite{nonlocal} were achieved via architectural innovation, increased compute, etc., our performance boost is purely from pre-training a simple architecture (R(2+1)D \cite{r2plus1D}) at scale. On Epic Kitchens action recognition challenge \cite{epicKitchens}, we achieve an mAP of $\boldsymbol{24.9\%}$ on unseen verb-noun pairs, an improvement of $\sim 8.5\%$ over the top entry in the leadership board at the time of this manuscript submission. 
\end{packed_enum}
%We do a careful in-depth analysis of various temporal aspects of videos. 
%On the other hand, while scaling to billions of images showed significant gains \cite{jft, uruImage}, we did not observe such boosts after about $10$ million pre-training videos.  
%\matt{At his point a natural question is how many distinct frames the image and video models each saw, and then there's a question of diversity of visual information which maybe we can't answer but should recognize.  I.e. are we actually exhausting the visual diversity in our label space?  It'll be easier to talk to this when some of the more recent experiments are done.}
%\note{@Matt: We are actually seeing improvement with more data. Do you still think there is value in comparing 3.5B images with the video model processing 492.5M videos in total of 32-frame input?}

%Given the well-known challenges in constructing large-scale fully-supervised video datasets, 



%what videos should one choose for pre-training from potentially billions of public web videos? Given a fixed training budget, should we choose - short videos having presumably good temporal localization of actions or longer videos which supply correlated side information and hence more content diversity?  
%Given fixed pre-training hours of video, should we choose a large number of short duration videos for pre-training or a smaller number of long videos. 




%We address this question in ths work and train video models on millions of videos using weak-supervision

%Similar to these, our approach also suffers from limited information, since hashtags mostly reflect objects 174 (nouns) and may not provide action-related information 175 contained in the video

%The effect of this temporal noise in web videos on the state-of-the-art video models \cite{r2plus1D, 3d1, 3d2, 3d3, nonlocal} when pre-trained at very large-scale is not immediately unclear. 
%\matt{Call out temporal localization here -- also mention that images are, by design, well localized 'good' frames, or people wouldn't post them, which is rather unlike a typical frame of video} 
%While all weakly-supervised datasets \cite{uruImage, jft, laurens} suffer from noisy, missing, or incorrect labels -- all due to lack of clear annotation supervision -- videos \textit{in-the-wild} face an additional challenge of the lack of \textit{temporal localization} of action labels. Specifically, real-world videos predominantly involve different composite actions with each action occupying only a very small fraction of the sequence. The extent of influence of this temporal noise on the state-of-the-art video models \cite{r2plus1D, 3d1, 3d2, 3d3, nonlocal} is not immediately unclear. 
%are available in abundance and therefore provide an opportunity as well as a challenge of choosing the right subset of them for training.

%Video action label space is fundamentally different from image tasks thus posing further challenges in terms of designing the right pre-training label space.


==> intro_old.tex <==
\section{Introduction}
Learning effective feature representations by training a model on large datasets in order to facilitate a variety of transfer learning tasks is a widely adopted practice in visual content understanding algorithms \cite{decaf, imagenetTransfer}. This transfer learning framework has shown clear performance benefits, especially when the target datasets are small \cite{segment, poseEstimation, oflow, posetrack, r2plus1D, nonlocal}. The role of large-scale data during pre-training towards improving the feature representations has been a long-standing question. Recently, in the context of images, studies \cite{uruImage, jft, laurens} have demonstrated that training on hundreds of millions (billions) of noisy web images with weak supervision significantly boosts the transfer learning performance. Despite these advances in the image domain, this question is yet to be answered for videos. \matt{This sentence is generic -- at this point the reader is probably wondering why they shouldn't expect every result to transfer directly.  This is an opportunity to call out what makes video interesting compared to images, e.g. "Video offers the additional dimensions of time and motion.  Is motion easy to learn given a good set of image features?  To what degree does temporal localization of labels matter?"}

In this work, we explore the feasibility of pre-training video models at extreme-scale using weak supervision for the task of action recognition from videos. Given the well-known challenges in constructing large-scale fully-supervised video datasets\footnote{For example, it was reported to take $\sim 80$ seconds to annotate a $10$ second long video in SOA dataset \cite{soa}, compared to identifying the presence of an object in an image in ImageNet \cite{imagenet}}, we argue that weakly-supervised pre-training at scale is even more vital for video tasks. Intuitively, a superior pre-trained model may hugely benefit transfer learning tasks on existing smaller video datasets. However, videos introduce an additional dimension of time and thus mandate joint encoding of spatial and motion information effectively in the model architectures \cite{r2plus1D, 3d1, 3d2, 3d3}. As a result, it is not immediately clear if the previous findings from weakly-supervised pre-training for images (effect of amount of data, label noise, long-tailed data distribution, etc.) would apply to video models at all. Furthermore, videos \textit{in-the-wild} are not temporally localized and the effect of this \textit{temporal noise} on large-scale pre-training is also not well-understood. Finally, action labels typically involve one (or more) objects and verbs to capture their interactions thus posing more challenges. This leads to other interesting yet unanswered questions, like the right way to leverage hashtags to construct action labels, the appropriate label space for actions during pre-training, etc. 

We address some of these open questions in this work. Our aim is to improve the learned video feature representations by focusing exclusively on training data instead of model-architecture design as is the status quo. Towards this end, we employ large-scale training of video models through \textit{weak} supervision. Specifically, we leverage over $65$ million public, user-generated videos from a social media website and use the associated hashtags as labels for pre-training. Despite the lack of clean labels, we observe that these videos and hashtags \textit{in-the-wild} enable pre-training of discriminative models. Unlike \underline{all} existing fully-supervised video datasets \cite{thumos, hmdb, kth, hollywood, ucf, kinetics, soa, momentsintime} which involved expensive annotation requirements, our training data is truly extensible to billion-scale without incurring any annotation costs. Below, we summarize our contributions:
\begin{packed_enum}
\vspace{-0.1in}
\item We show that for videos, large-scale data, despite not providing strong supervision, tremendously helps models of varied capacities in learning better features. Fine-tuning our largest model pre-trained on over $65M$ unique videos achieves a top-1 video accuracy of $\boldsymbol{80.59\%}$ on Kinetics which is a $2.9\%$ boost over the previous state-of-the-art \cite{nonlocal} (Sec. \ref{sec:sota}).  \matt{It's worth remarking that NLNN achieves gains via architectural innovation and increased compute, whereas the big data gains come from simpler madels and are likely complementary.} On Epic Kitchens action recognition challenge \cite{epicKitchens}, we achieve an mAP of $\boldsymbol{24.9\%}$ on unseen action classes \matt{"unseen action classes" sounds really weird unless you know the challenge -- maybe write "unseen verb-noun pairs" or something to help the unfamiliar reader}, an improvement of around $8.5\%$ over the top entry in the leadership board at the time of the submission of this manuscript. Thus, our experiments clearly demonstrate that content diversity and scale outdo label and data noise.
\item We perform a series of ablation studies, such as the effect of pre-training data size, model capacity, label space, and so on, and make several interesting observations. For instance, similar to previous studies on images \cite{uruImage}, we find that both increasing the model capacity (Sec. \ref{sec:capacity}) and matching the label space of pre-training and target datasets (Sec. \ref{sec:labelType}) improves performance on target tasks. On the other hand, while scaling to billions of images showed significant gains \cite{jft, uruImage}, we did not observe such boosts after about $10$ million pre-training videos.  \matt{At his point a natural question is how many distinct frames the image and video models each saw, and then there's a question of diversity of visual information which maybe we can't answer but should recognize.  I.e. are we actually exhausting the visual diversity in our label space?  It'll be easier to talk to this when some of the more recent experiments are done.}
\item We do an in-depth analysis of various temporal aspects of videos. Given the established leaping benefits from pre-training on billions of images \cite{uruImage}, we investigate the true value of pre-training using video data. We show that it is necessary to pre-train using videos as opposed to images followed by inflation~\cite{i3d} to achieve better performance when operating at scale (Sec. \ref{sec:image2video}). We also study the effect of pre-training on shorter and longer duration videos to understand the effect of temporal noise and diversity (Sec. \ref{sec:vidLengths}) \note{Report observations when we have results}.
\end{packed_enum}

%%%% == Deepti %%%%
%Learning effective feature representations by training a model on large datasets so as to perform well on a variety of transfer learning tasks is a widely adopted practice in visual content understanding algorithms \cite{decaf, imagenetTransfer}. This transfer learning framework has shown clear performance benefits on a variety of video tasks, especially when the target datasets are small \cite{oflow, posetrack, r2plus1D, nonlocal}. 
%There has been a long standing question about the importance of large-scale data in learning better visual representations during pre-training. Recently, this has been explored in the context of images in a few studies \cite{uruImage, jft, laurens} demonstrating that training on billions of noisy web images significantly boosts the transfer learning performance. However, this continues to remain an open question in videos 
%primarily because it is very expensive and laborious to construct video datasets compared to images limiting our ability to scale to fully-supervised models. Furthermore, videos encode information sequentially and thus mandate encoding of temporal and motion information effectively. Thus, simple extension of image models to video tasks is not sufficient \cite{karpathy}. Training video models that jointly capture spatial and temporal information is essential but also orders of magnitudes challenging compared to image models. 
%In this work, we aim to improve the learned video feature representations by focusing exclusively on training data instead of model-architecture design as is the status quo. Towards this end, we employ large-scale training of video models through \textit{weak} supervision. Specifically, we leverage millions of public, user-generated videos from Instagram and the metadata associated with them such as hashtags, video captions, and so on. Unlike \underline{all} existing fully-supervised video datasets \note{cite all works}, our training data is truly extensible to billion-scale without incurring any annotation costs. This is because, we pose the pre-training task as predicting the hashtags which are readily available. Thus, despite the lack of strong labels, this data can enable pre-training of discriminative models, followed by fine-tuning on any target task of choice. However, as has been observed in the precursory efforts using large-scale, weakly-supervised image data \cite{jft, uruImage}, the labels are very noisy, often missing, or incorrect. Furthermore, the data distribution is long-tailed further posing a challenge to train models at scale. 
%Below, we describe our attack on the difficult problem of million-scale pre-training of video models and summarize our contributions:
% \begin{packed_enum}
% %\vspace{-0.15in}
% \item \textbf{Scale matters:} Our primary observation is that large-scale data, despite not providing strong supervision, tremendously helps models of varied capacities in learning better feature representations as observed in the huge boosts in the performance across all target datasets (Sec. \ref{sec:sota}). Our experiments prove that content diversity and scale outdo label and data noise.
% \item \textbf{More data and larger models imply better performance:} We found that performance increases as we increase the amount of training data and then plateaus after a point (after about $10M$ datapoints, see Sec. \ref{sec:datapoints}). We also found that higher capacity models tended to over-fit less and benefit more from large-scale data (Sec. \ref{sec:capacity}).
% \note{report the boost when using 65M between 34 and 101 layers}. This may indicate a need to increase the representational capacity of the networks to truly benefit from million-scale data. 
% \item \textbf{Nature of hashtags matters:} We found that target tasks benefit when noisy hashtags supplying weak supervision strongly correlate with the target labels (Sec. \ref{sec:labelType}) \note{report the final boost in performance}. This result corroborates the observations made in the context of images in \cite{uruImage}. 
% \item \textbf{Motion matters at scale:} Given the leaping benefits from billion-scale images \cite{uruImage}, we investigated the true value in using video data during pre-training. We found that pre-training a $3D$ convolutional model on video data yields significant boosts compared to a $2D$ convolutional model on million-scale image data thus underscoring the value of modeling motion.
% \item \textbf{State-of-the-art results:} Our largest model is trained on over $65M$ unique videos and uses over $10,000$ action-driven hashtags for weak supervision. Upon fine-tuning this model and no additional bells and whistles, we achieved a top-1 video accuracy of $\boldsymbol{80.59\%}$ on Kinetics which is a total of $2.9\%$ boost over the previous state-of-the-art \cite{nonlocal}. We achieved outstanding performance on many other target datasets which we report in Sec. \ref{sec:sota}.
% \note{Report performance on all target datasets.}
% \end{packed_enum}
%aim is to advance the state of video understanding. 

==> intro_old1.tex <==
\section{Introduction}
Learning effective feature representations by training a model on large datasets in order to facilitate a variety of transfer learning tasks is a widely adopted practice in visual content understanding algorithms \cite{decaf, imagenetTransfer}. This transfer learning framework has shown clear performance benefits, especially when the target datasets are small \cite{segment, poseEstimation, oflow, posetrack, r2plus1D, nonlocal}. The role of large-scale data during pre-training towards improving the feature representations has been a long-standing question. Recently, in the context of images, studies \cite{uruImage, jft, laurens} have demonstrated that training on hundreds of millions (billions) of noisy web images with weak supervision significantly boosts the transfer learning performance. We argue that addressing this question for videos is even more challenging. While web images suffer from label noise, \textit{in-the-wild} videos additionally have to also deal with 
the lack of temporal localization of labels thereby leading to temporal noise. (Presence / absence of the action, incorrect action label, where in the video is the labeled action). 

Thus, pre-training at scale using videos share a few challenges with that of images. Not sure if they will directly translate thus making it important to revisit this question for videos. Going beyond this, videos introduce further challenges - eg: what should the label space contain - focus on nouns or verbs? How does pre-training on variety of concepts help?

What kind of videos should we choose - short videos succinctly capturing videos vs. long videos which supply correlated side information hence more diversity?  Should we pre-train on videos at all, given the leaping benefits from images?


Despite these advances in the image domain, this question is yet to be answered for videos.
Given that videos offer the additional dimension of time and motion, it is natural to question: Is motion easy to learn given a good set of image features? Do the previous findings from weakly-supervised pre-training for images (effect of amount of data, label noise, long-tailed data distribution, etc.) also apply to video models that jointly encode spatial and motion information \cite{r2plus1D, 3d1, 3d2, 3d3}? Furthermore, videos \textit{in-the-wild} are not temporally localized and the effect of this \textit{temporal noise} on large-scale pre-training is also not well-understood. Finally, action labels typically involve one (or more) objects and verbs to capture their interactions thus posing more challenges. This leads to other interesting yet unanswered questions, like the right way to leverage hashtags to construct action labels, the appropriate label space for actions during pre-training, etc.}

In this work, we explore the feasibility of pre-training video models at extreme-scale using weak supervision for the task of action recognition from videos. Given the well-known challenges in constructing large-scale fully-supervised video datasets\footnote{For example, it was reported to take $\sim 80$ seconds to annotate a $10$ second long video in SOA dataset \cite{soa}, compared to identifying the presence of an object in an image in ImageNet \cite{imagenet}}, we argue that weakly-supervised pre-training at scale is even more vital for video tasks. Intuitively, a superior pre-trained model may hugely benefit transfer learning tasks on existing smaller video datasets. Thus, our aim is to improve the learned video feature representations by focusing exclusively on training data instead of model-architecture design as is the status quo. In our very large-scale weakly-supervised pre-training setup, we leverage over $65$ million public, user-generated videos from a social media website and use the associated hashtags as labels for pre-training. Despite the lack of clean labels, we observe that these videos and hashtags \textit{in-the-wild} enable pre-training of discriminative models. Unlike \underline{all} existing fully-supervised video datasets \cite{thumos, hmdb, kth, hollywood, ucf, kinetics, soa, momentsintime} which involved expensive annotation requirements, our training data is truly extensible to billion-scale without incurring any annotation costs. Below, we summarize our contributions:
\begin{packed_enum}
\vspace{-0.1in}
\item We show that for videos, large-scale data, despite not providing strong supervision, tremendously helps models of varied capacities in learning better features. Fine-tuning our largest model pre-trained on over $65M$ unique videos achieves a top-1 video accuracy of $\boldsymbol{80.49\%}$ on Kinetics which is a $2.8\%$ boost over the previous state-of-the-art \cite{nonlocal} (Sec. \ref{sec:sota}).\textcolor{red}{While the performance gains in \cite{nonlocal} were achieved via architectural innovation, increased compute, etc. our performance boost is purely from training a simpler architecture on very large-scale dataset.}
\matt{It's worth remarking that NLNN achieves gains via architectural innovation and increased compute, whereas the big data gains come from simpler madels and are likely complementary.}
On Epic Kitchens action recognition challenge \cite{epicKitchens}, we achieve an mAP of $\boldsymbol{24.9\%}$ on \textcolor{red}{unseen verb-noun pairs} \matt{"unseen action classes" sounds really weird unless you know the challenge -- maybe write "unseen verb-noun pairs" or something to help the unfamiliar reader}, an improvement of around $8.5\%$ over the top entry in the leadership board at the time of the submission of this manuscript. Thus, our experiments clearly demonstrate that content diversity and scale outdo label and data noise.
\item We perform a series of ablation studies, such as the effect of pre-training data size, model capacity, label space, and so on, and make several interesting observations. For instance, similar to previous studies on images \cite{uruImage}, we find that increasing the number of training videos (Sec. \ref{sec:datapoints}), increasing the model capacity (Sec. \ref{sec:capacity}), and matching the label space of pre-training and target datasets (Sec. \ref{sec:labelType}) improve performance on target tasks. 
%On the other hand, while scaling to billions of images showed significant gains \cite{jft, uruImage}, we did not observe such boosts after about $10$ million pre-training videos.  
\matt{At his point a natural question is how many distinct frames the image and video models each saw, and then there's a question of diversity of visual information which maybe we can't answer but should recognize.  I.e. are we actually exhausting the visual diversity in our label space?  It'll be easier to talk to this when some of the more recent experiments are done.}
\note{@Matt: We are actually seeing improvement with more data. Do you still think there is value in comparing 3.5B images with the video model processing 492.5M videos in total of 32-frame input?}
\item We do an in-depth analysis of various temporal aspects of videos. Given the established leaping benefits from pre-training on billions of images \cite{uruImage}, we investigate the true value of pre-training using video data. We show that it is necessary to pre-train using videos as opposed to images followed by inflation~\cite{i3d} to achieve better performance when operating at scale (Sec. \ref{sec:image2video}). We also study the effect of pre-training on shorter and longer duration videos to understand the effect of temporal noise and diversity (Sec. \ref{sec:vidLengths}) \note{Report observations when we have results}.
\end{packed_enum}

%%%% == Deepti %%%%
%Learning effective feature representations by training a model on large datasets so as to perform well on a variety of transfer learning tasks is a widely adopted practice in visual content understanding algorithms \cite{decaf, imagenetTransfer}. This transfer learning framework has shown clear performance benefits on a variety of video tasks, especially when the target datasets are small \cite{oflow, posetrack, r2plus1D, nonlocal}. 
%There has been a long standing question about the importance of large-scale data in learning better visual representations during pre-training. Recently, this has been explored in the context of images in a few studies \cite{uruImage, jft, laurens} demonstrating that training on billions of noisy web images significantly boosts the transfer learning performance. However, this continues to remain an open question in videos 
%primarily because it is very expensive and laborious to construct video datasets compared to images limiting our ability to scale to fully-supervised models. Furthermore, videos encode information sequentially and thus mandate encoding of temporal and motion information effectively. Thus, simple extension of image models to video tasks is not sufficient \cite{karpathy}. Training video models that jointly capture spatial and temporal information is essential but also orders of magnitudes challenging compared to image models. 
%In this work, we aim to improve the learned video feature representations by focusing exclusively on training data instead of model-architecture design as is the status quo. Towards this end, we employ large-scale training of video models through \textit{weak} supervision. Specifically, we leverage millions of public, user-generated videos from Instagram and the metadata associated with them such as hashtags, video captions, and so on. Unlike \underline{all} existing fully-supervised video datasets \note{cite all works}, our training data is truly extensible to billion-scale without incurring any annotation costs. This is because, we pose the pre-training task as predicting the hashtags which are readily available. Thus, despite the lack of strong labels, this data can enable pre-training of discriminative models, followed by fine-tuning on any target task of choice. However, as has been observed in the precursory efforts using large-scale, weakly-supervised image data \cite{jft, uruImage}, the labels are very noisy, often missing, or incorrect. Furthermore, the data distribution is long-tailed further posing a challenge to train models at scale. 
%Below, we describe our attack on the difficult problem of million-scale pre-training of video models and summarize our contributions:
% \begin{packed_enum}
% %\vspace{-0.15in}
% \item \textbf{Scale matters:} Our primary observation is that large-scale data, despite not providing strong supervision, tremendously helps models of varied capacities in learning better feature representations as observed in the huge boosts in the performance across all target datasets (Sec. \ref{sec:sota}). Our experiments prove that content diversity and scale outdo label and data noise.
% \item \textbf{More data and larger models imply better performance:} We found that performance increases as we increase the amount of training data and then plateaus after a point (after about $10M$ datapoints, see Sec. \ref{sec:datapoints}). We also found that higher capacity models tended to over-fit less and benefit more from large-scale data (Sec. \ref{sec:capacity}).
% \note{report the boost when using 65M between 34 and 101 layers}. This may indicate a need to increase the representational capacity of the networks to truly benefit from million-scale data. 
% \item \textbf{Nature of hashtags matters:} We found that target tasks benefit when noisy hashtags supplying weak supervision strongly correlate with the target labels (Sec. \ref{sec:labelType}) \note{report the final boost in performance}. This result corroborates the observations made in the context of images in \cite{uruImage}. 
% \item \textbf{Motion matters at scale:} Given the leaping benefits from billion-scale images \cite{uruImage}, we investigated the true value in using video data during pre-training. We found that pre-training a $3D$ convolutional model on video data yields significant boosts compared to a $2D$ convolutional model on million-scale image data thus underscoring the value of modeling motion.
% \item \textbf{State-of-the-art results:} Our largest model is trained on over $65M$ unique videos and uses over $10,000$ action-driven hashtags for weak supervision. Upon fine-tuning this model and no additional bells and whistles, we achieved a top-1 video accuracy of $\boldsymbol{80.59\%}$ on Kinetics which is a total of $2.9\%$ boost over the previous state-of-the-art \cite{nonlocal}. We achieved outstanding performance on many other target datasets which we report in Sec. \ref{sec:sota}.
% \note{Report performance on all target datasets.}
% \end{packed_enum}
%aim is to advance the state of video understanding. 

==> oldexpts.tex <==
\section{Experiments} \label{sec:experiments}
% \begin{figure*}[t]
% \begin{center}$
% \begin{array}{cc}
% \includegraphics[width=2.6in, height=2.1in]{figures/fig2a_kinetics} & 
% \includegraphics[width=2.6in, height=2.1in]{figures/fig2b_kitchens} \\
% \end{array}$ 
% \caption{\footnotesize{Illustrating the effect of increasing the number of pre-training videos from $500K$ videos to $65M$. The baseline (training from scratch) is indicated in blue. Network architecture: R(2+1)D-34. Best viewed in color.}}
% \vspace{-0.15in}
% \label{fig:dataPoints}
% \end{center}
% \end{figure*}
\subsection{Evaluation Setup} 
As mentioned, a pre-trained model serves as a sophisticated initializer of the video model parameters and we fine-tune it on a number of target datasets. To illustrate the benefit of using millions of videos, we also pre-trained on benchmark datasets such as Sports-1M \cite{sports1m}, Kinetics \cite{kinetics} as strong baselines. As in \cite{uruImage}, we report the performance in two scenarios:
\begin{packed_enum}
\vspace{-0.07in}
\item \textbf{{Full-finetuning approach}} involves first replacing the hashtag-specific layer in the pre-trained model with a randomly initialized and fully-connected layer. The number of output units in this layer match the number of classes in each target dataset. This model would then be trained end-to-end for much fewer epochs on the target dataset to adapt to the target task. In order to find the best hyper-parameters (learning rate, schedule, etc.), we do a grid search on a small validation data held out from the training set. The hyper parameters per experiment and target dataset are in the supplementary material. 
\item \textbf{fc-only finetuning approach} involves extracting features from the final fully-connected layer of a pre-trained model and training a logistic regressor on each target dataset. 
\vspace{-0.1in}
\end{packed_enum}
While the full-finetuning approach has the disadvantage that it can potentially mask the absolute effect of pre-training if the target dataset is large, fc-only approach does not suffer from this consequence. In both evaluation methods, we report video \textit{top-1 accuracy} for multi-class and \textit{mAP} for multi-label target datasets. During testing, center crops of $10$ clips uniformly sampled from each test video are considered, and the average of these $10$ clip predictions are used to obtain the final video-level prediction. 

Below, we report our analysis on three broad aspects of very large-scale training: (a) the effect of scale - e.g., model capacity and pre-training data size (b) the design of the pre-training label space, and (c) temporal properties of videos.
\begin{figure}
\begin{center}$
\begin{array}{cc}
\includegraphics[width=1.6in, height=1.4in]{figures/datapoints_fig1a} & 
\includegraphics[width=1.6in, height=1.4in]{figures/datapoints_fig1b} \\
\end{array}$ 
\caption{\footnotesize{Illustrating the effect of increasing the number of pre-training videos from $500K$ videos to $65M$. The baseline (training from scratch) is indicated in blue. Best viewed in color.}}
\vspace{-0.2in}
\label{fig:dataPoints}
\end{center}
\end{figure}
\subsection{Does extreme-scale help?}
\subsubsection{Effect of the amount of pre-training data} \label{sec:datapoints}
To understand this question, we pre-train on different amounts of training data by constructing $6$ different data subsets -- \WStwo{Kinetics}{500K}, \WStwo{Kinetics}{1M}, \WStwo{Kinetics}{5M}, \WStwo{Kinetics}{10M}, \WStwo{Kinetics}{19M}, and \WStwo{Kinetics}{65M} respectively. $6$ R(2+1)D-34 models were independently trained on these datasets on an input of $8$-frames per video and a mini-batch size of $16$.\\
\textbf{Key takeaways:} Figure \ref{fig:dataPoints} reports the performance after finetuning on Kinetics and Epic-Kitchens, from which we may conclude that:
\begin{packed_enum}
\vspace{-0.1in}
\item Pre-training R(2+1)D-34 yields a video top-1 accuracy of $74.82\%$, which is an improvement of $\boldsymbol{\sim~7.9\%}$ compared to training the same model from scratch on Kinetics ($66.94\%$). This significant boost in accuracy clearly highlights the benefit of training video models on very large-scale data.
\item The classification performance steadily increases with the amount of pre-training data. In full-finetuning approach, the performance appears to saturate after about $10M$ datapoints as there is a marginal improvement of $\sim0.3\%$ in the top-1 accuracy when \WStwo{Kinetics}{65M} was used compared to \WStwo{Kinetics}{10M}. However, using fc-only approach, we observe that accuracy continues to improve, indicating that the model continues to learn better feature representations with more pre-training data, which is being masked due to full-finetuning.
\item All the aforementioned observations are generalizable to Epic-Kitchens too as reported in Fig. \ref{fig:dataPoints} (b). \note{Report the improvement in the baseline for Kitchens.}
\end{packed_enum}
\subsubsection{Effect of model capacity in million-scale training framework} \label{sec:capacity}
To closely understand how pre-training on large-scale data varies with the capacity of video models, we trained $4$ different R(2+1)D-d models described earlier, where $d = \{18, 34, 101, 152\}$. Each model was trained on the exact same pre-training dataset \WStwo{Kinetics}{65M}, on an input of $32$-frames per video, and a mini-batch size of $6$. On Kinetics (Table \ref{tbl:depthKinetics}), we may observe that the performance consistently improves with the increase in model capacity, yielding a total boost of $3\% - 4\%$. By comparison, when training from scratch on Kinetics, the top-1 accuracy does not significantly improve with model capacity. On the other hand, on Epic-Kitchens (Table \ref{tbl:depthKitchens}), while the performance initially improves, R(2+1)D-152 results in a drop of about $\sim1\%$ compared to R(2+1)D-101. We suspect that this is due to over-fitting and that the 152-layer network when pre-trained on \WStwo{Kinetics}{65M} may be unnecessarily complex for this relatively small, domain-specific dataset. This opens a future direction to be explored -- modifying large-scale, weakly supervised pre-training to better suit a variety of target datasets that differ in their size and action-diversity.

%This high performance boost when higher capacity models are coupled with large-scale data may also support a hypothesis that models larger than R(2+1)D-152 could potentially further benefit from pre-training on millions of videos. We hope that this valuable finding will further inspire the community to explore high capacity spatio-temporal video network designs.
\begin{table}[t]
%\vspace{-0.07in}
\footnotesize
\setlength\extrarowheight{1.2pt}
\centering
\begin{center}
\begin{tabular}{|P{1.7cm}|P{1.cm}|P{1.cm}|P{1.cm}|}
\hline
 Model &  full-ft & fc-only & baseline \\
\hhline{|=|=|=|=|}
R(2+1)D-18 & 75.96 & 73.4 & 69.34 \\
\hline
R(2+1)D-34 & 78.24 & 75.38 & 69.56 \\
\hline
R(2+1)D-101 & 79.13 & 77.18 & 71.71 \\
\hline
R(2+1)D-152 & 79.54 & 77.26 & 72.02 \\
\hline
\end{tabular}
\end{center}
\vspace{-0.1in}
\caption{\footnotesize{Top-1 accuracy when pre-trained models of varied capacities are finetuned on Kinetics.}}
\vspace{-0.15in}
\label{tbl:depthKinetics}
\end{table}
\begin{table}[t]
%\vspace{-0.07in}
\footnotesize
\setlength\extrarowheight{1.2pt}
\centering
\begin{center}
\begin{tabular}{|P{1.7cm}|P{1.cm}|P{1.cm}|P{1.cm}|}
\hline
 Model &  full-ft & fc-only & baseline \\
\hhline{|=|=|=|=|}
R(2+1)D-18 & 20.83 & 6.48 & 14.82 \\
\hline
R(2+1)D-34 & 22.39	& 8.6 & 15.18 \\
\hline
R(2+1)D-101 & 24.87	& 8.17 & 17.14 \\
\hline
R(2+1)D-152 & 23.66	& 7.01 & 17.76 \\
\hline
\end{tabular}
\end{center}
\vspace{-0.1in}
\caption{\footnotesize{mAP when pre-trained models of varied capacities are finetuned on Epic-Kitchens.}}
\vspace{-0.15in}
\label{tbl:depthKitchens}
\end{table}
\subsection{What makes a pre-training label space effective?} \label{sec:labelEffect}
\begin{figure*}[t]
\begin{center}$
\begin{array}{cccc}
\includegraphics[width=1.6in, height=1.2in]{figures/typeLabels_figa} & 
\includegraphics[width=1.6in, height=1.2in]{figures/typeLabels_figb} &
\includegraphics[width=1.6in, height=1.2in]{figures/typeLabels_figc} & 
\includegraphics[width=1.6in, height=1.2in]{figures/typeLabels_figd} \\
\end{array}$ 
\caption{\footnotesize{(a) Top-1 accuracy on Kinetics and (b)-(d) mAP on the three Epic-Kitchens tasks after fc-only finetuning, when different source label sets are used (indicated in the legend). The results indicate that target tasks benefit the most when their labels overlap with the source hashtags. Best viewed in color.}}
\vspace{-0.25in}
\label{fig:labelType}
\end{center}
\end{figure*}
\subsubsection{Effect of the nature of pre-training labels}\label{sec:labelType} 
\begin{table}[t]
%\vspace{-0.15in}
\scriptsize
\setlength\extrarowheight{1.2pt}
\centering
\begin{center}
\begin{tabular}{|P{1.4cm}|P{1.2cm}|P{0.9cm}|P{1.5cm}|P{0.9cm}|}
\hline
 &  \WSone{Kinetics} (359) & \WSone{Verb} (438) & \WSone{Verb+Noun} (10563) & \WSone{Noun} (1428)\\
\hhline{|=|=|=|=|=|}
Kinetics (400) & 1 & 0.9 & 0.03 & 0.04 \\
\hline
Epic-Kitchens & &  & &  \\
\hline
\end{tabular}
\end{center}
\vspace{-0.1in}
\caption{\scriptsize{Percentage of target labels that overlap with pre-training labels.}}
\vspace{-0.1in}
\label{tbl:source-target-overlap}
\end{table}
Next, we considered the question: what constitutes a valuable pre-training label space for achieving superior transfer learning performance? To address this, we considered two scenarios - when hashtags a) do overlap and b) do not overlap with the target dataset's label space. Towards this end, we fixed the number of unique videos to sample to be $19M$, varied the seed labels, and constructed \WStwo{Kinetics}{19M}, \WStwo{Verb}{19M}, \WStwo{Noun}{19M}, and \WStwo{Verb+Noun}{19M} as our pre-training datasets (more details on the datasets in Sec. \ref{sec:igdataset}). As a way to quantify the label space overlap, we identified the verbs and the nouns from all target and source labels and reported the percentage of matches between them in Table \ref{tbl:source-target-overlap}. Each R(2+1)D-34 model was trained on an input of $32$-frames per video and a mini-batch size of $6$ videos. To distinctly highlight the effect of pre-training label space, we evaluate using fc-only finetuning approach. We note that we observed similar trends when we employed full-finetuning, which we report in the supplementary material due to space constraints. \\
\textbf{Key takeaways:} From Fig. \ref{fig:labelType}, we may observe that for each target dataset, the source dataset whose labels overlap the most with it yield maximum performance. For instance, for Kinetics we see an improvement of \textit{at least} $\sim 5\%$, when \WStwo{Kinetics}{19M} was used for pre-training, compared to other pre-training datasets (Fig. \ref{fig:labelType}(a)). Pre-training on \WStwo{Noun}{19M} benefits the noun prediction task the most while \WStwo{Verb}{19M} helps the verb prediction task the most (at least 1.5\% in both cases, Fig. \ref{fig:labelType}(b)). Thus, in a transfer learning scenario, it may be efficient to choose those pre-training hashtags that most overlap with the target label space for achieving maximum performance gains.
\subsubsection{Effect of the number of pre-training labels}\label{sec:numLabels}
\begin{figure}[t]
\vspace{-0.1in}
\begin{center}$
\begin{array}{cc}
\includegraphics[width=1.6in, height=1.4in]{figures/numlabels_a} & 
\includegraphics[width=1.6in, height=1.4in]{figures/numlabels_b} \\
\end{array}$ 
\caption{\footnotesize{Top-1 accuracy on Kinetics when pre-training on different number of hashtags. Note that the source datasets used in panels (a) and (b) are different, hence the results are not comparable.\note{increase fontsize.}}}
\vspace{-0.25in}
\label{fig:numLabels}
\end{center}
\end{figure}
In Sec. \ref{sec:datapoints}, we studied how varying the number of pre-training videos for a fixed source label space effects the transfer learning performance. In this section, we investigated the reverse scenario, i.e., vary the number of pre-training labels while keeping the number of videos fixed.\\ 
\textbf{Experiment setup \#1:} For this experiment, we considered \WStwo{Verb+Noun}{25M} as our candidate pre-training dataset, which has a total of $10,653$ action labels and $25M$ videos. We chose this specific dataset only because of it's large action label space which enabled us to effectively vary the number of pre-training labels and study its effect on transfer learning. Note that \cite{imagenetTransfer} reports a similar analysis for image-based tasks by systematically traversing the WordNet hierarchy and varying the number of labels from $1000$ to $127$. However, none of our source label sets (Sec. \ref{sec:datasetprop}) have an analogous video-actions taxonomy to traverse and systematically generate different granularities of action labels. Therefore, we randomly sub-sampled different number of labels from the full set of $10,653$ labels all the way to $675$ labels \footnote{We did not have enough training videos, i.e., at least $1M$ for number of labels fewer than $675$.} in steps of $0.5$, resulting in the following label sets: $L_{10K}$, $L_{5400}$, $L_{2700}$, $L_{1350}$, $L_{675}$, where the subscript denotes the total number of labels in that label set $L$. Label sampling was done such that the $L_{675} \subset L_{1350} \subset L_{2700} \subset L_{5400} \subset L_{10K}$. We pre-trained $5$ separate R(2+1)D-34 models on videos associated with these label sets by keeping the number of videos fixed at $1M$, input clip-length of $8$-frames, and a mini-batch size of $16$.

From Fig. \ref{fig:numLabels} (a), we may observe that, upon full-finetuning on Kinetics, there is an improvement of about $~1\%$ between $L_{675}$ and $L_{1350}$, and the performance saturates after that (only $~0.2\%$ improvement). In the fc-only finetuning scenario, we also observe an improvement of $~7\%$ between $L_{675}$ and $L_{1350}$ and a further improvement of $2\%$  when compared to $L_{2700}$. Following this, the performance tends to saturate, perhaps due to underfitting of the model. \\
\noindent \textbf{Experiment setup \#2:} To further understand the effect when the number of pre-training labels are fewer than the target labels (i.e, \textless $400$ for Kinetics), we considered \WStwo{Kinetics}{19M} as our pre-training dataset only because this dataset supplied sufficient videos for training. Once again, we sampled labels as described above in steps of $0.5$, resulting in sets: $L_{360}$, $L_{180}$, $L_{90}$, $L_{45}$, and $L_{20}$ such that $L_{20} \subset L_{45} \subset L_{90} \subset L_{180} \subset L_{360}$. As was done earlier, $5$ different models were trained on $1M$ unique videos associated with these label sets. From Fig. \ref{fig:numLabels} (b), we may observe that the performance upon full-finetuning gradually declines by about $1\% - 2\%$ as we reduce the labels in steps of $0.5$. There is a significant drop of $\sim 6\%$ between $L_{360}$ and $L_{20$. The drop in the performance is more severe when we perform fc-only finetuning ($15.35\%$ vs. $60.76\%$).\\ 
\textbf{Key takeaway:} These two experiments suggest that more diverse visual pre-training labels generally lead to the model learning improved feature representations, with diminishing gains after about $2700$ labels for Kinetics. Also, there is a decline in the performance when the pre-training labels are very few labels (eg: $20$), when compared to training a model from scratch on all $400$ Kinetics labels ($66.94\%$ top-1 accuracy). It will be interesting to investigate the interplay between increasing number of labels that are semantically very similar or dissimilar to target labels in future.
\subsection{Exploring the temporal considerations of video} \label{sec:temporal}
\subsubsection{Robustness to temporal noise} \label{sec:vidLengths}% Effect of vid. durations
As mentioned in Sec. \ref{sec:igdataset}, our dataset inherently has large amounts of \textit{temporal noise} as video lengths range from $1$ -- $60$ seconds and no manual cleaning was undertaken. This high temporal diversity leads to the following questions:\\
(q1) Short videos are more likely to succinctly capture an action compared to longer ones. Given this, how does pre-training on short vs long videos effect transfer learning?  \\
(q2) Due to temporal jittering, in each epoch, a clip from a random location of the input video would be sampled. Thus, longer videos are likely to supply a lot more content variety compared to short videos. Is this randomly sampled content strongly-correlated with the labeled action or is it noise? \\
To answer these questions, we constructed two datasets from \WStwo{Kinetics}{65M} on a fixed label space: \\
(i) $short\_vids$: videos of lengths between $1$ -- $5$ seconds.\\
(ii) $long\_vids$: videos of lengths between $55$ -- $60$ seconds.\\
We sampled $5M$ unique videos from $short\_vids$ and $long\_vids$ independently and trained two separate models (say $Short\_5M$ and $Long\_5M$) on them. As mentioned above in (q2), the model $Long\_5M$ is likely to be presented with much more unique content than $Short\_5M$. Thus, for a fair comparison, we trained another model by sampling only $500K$ unique videos from $long\_vids$ ($Long\_500K$). Further, to understand the issue of localized actions as mentioned in (q1), we consider the same set of $5M$ unique videos as were used by $Long\_5M$, but restrict the temporal jittering only to the \textit{center portion} of each input video. That is, for a $60$ second long input video, in each epoch, a random clip from the center portion, i.e., $28$ -- $32$ seconds is sampled. We denote the model trained in this setting as $Long-center\_5M$. This setting also leads to a further fairer comparison of the models $Long-center\_5M$ and $Short\_5M$. Each R(2+1)D-34 model was independently trained on an input of $8$-frames per video and a mini-batch size of $16$.\\
\textbf{Key takeaways:} \note{talk about results}. These results corroborate our hypothesis that short videos suffer from relatively less temporal noise compared to longer videos, thereby leading to faster convergence during pre-training. 
\begin{table}
\footnotesize
\setlength\extrarowheight{1.2pt}
\centering
\begin{center}
\begin{tabular}{|P{2.4cm}|P{3.4cm}|P{1cm}|}
\hline
 &  Temporal jittering strategy & Top-1 accuracy\\
\hhline{|=|=|=|}
$Short\_5M$ & uniformly random throughout & 56.87\\
\hline
$Long\_5M$ & uniformly random throughout & 60.31\\
\hline
$Long\_500K$ & uniformly random throughout & 50.6\\
\hline
$Long-center\_5M$ & uniformly random in the center $4$ second window & 50.78
\\
\hline
\end{tabular}
\end{center}
\vspace{-0.1in}
\caption{\footnotesize{Video top-1 accuracy when R(2+1)D-34 is pre-trained on $4$ different datasets constructed from $short\_vids$ and $long\_vids$, followed by fc-only finetuning on target dataset Kinetics.}}
\vspace{-0.2in}
\label{tbl:vidLengths}
\end{table}
\begin{table*}[t]
\footnotesize
\setlength\extrarowheight{1.2pt}
\centering
\begin{center}
\begin{tabular}{|P{2.1cm}|P{2.5cm}|P{1.9cm}|P{2.5cm}|P{1.6cm}|P{1.9cm}|}
\hline
 Input dataset &  Pre-training Input & Pre-train model  & Test strategy & Test input & Top-1 accuracy\\
\hhline{|=|=|=|=|=|=|}
\WS{I}{K}{19M} & Image & R2D-18 & Inflate to R3D-18 & Video & 66.99 \\
\hline
\WStwo{Kinetics}{19M} & Random video frame & R2D-18 & Inflate to R3D-18  & Video & 67.45 \\
\hline
\WS{I}{K}{250M} & Image & R2D-18 & Inflate to R3D-18 & Video & 66.97 \\
\hline
ImageNet & Image & R2D-18 & Inflate to R3D-18 & Video & 66.5 \\
\hhline{|=|=|=|=|=|=|}
Kinetics & Video (8 frames) & R3D-18 & None & Video & 65.61 \\
\hline
\WStwo{Kinetics}{19M} & Video (8 frames) & R3D-18 & None & Video & \textbf{71.73} \\
\hline
\end{tabular}
\end{center}
\vspace{-0.05in}
\caption{\footnotesize{Experiment setup for understanding the benefit of using images vs. videos for million-scale pre-training.}}
\vspace{-0.1in}
\label{tbl:image2video1}
\end{table*}
\subsubsection{Do we need to pre-train on video data in a million-scale framework?} \label{sec:image2video}
Given the breakthrough in object classification with billion-scale image pre-training \cite{uruImage}, it is natural to question the true value in pre-training using video data and spatio-temporal convolutions. Though most leading action recognition models are pre-trained on ImageNet and operate on individual video frames thereby ignoring the temporal structure \cite{sports1m, i3d, nonlocal}, recent work by Tran \textit{et.al} \cite{r2plus1D} underscores the benefit of temporal modeling. We compare these two contrary approaches at scale and address the following questions: \\
(a) How well do the $2D$ convolutional models pre-trained on images compete with the $3D$ convolutional models pre-trained on videos at scale? \\
(b) The sequential nature of video data makes it compositionally different from images. Thus, is there any difference in performance when static video frames are considered for pre-training 2D models compared to images?

Towards this end, we first pre-train an $18$ layer $2D$ deep residual model R2D \cite{residual} from scratch on different types of $2D$ data (image/single video frames). We then \textit{inflate} \cite{i3d} this model to $R3D$ to facilitate evaluation on 3D data (videos). This is compared to a clip-based model $R3D$ (described in \cite{r2plus1D}) trained from scratch on video data and evaluated on videos. We summarize these different training setups with varied input data in Table \ref{tbl:image2video1}.

In this section, we use a notation $IG-{modality}-{source}-{size}$, where \textit{modality} denotes if it is an image or a video dataset, \textit{source} and \textit{size} denote the seed label space and the training data size as was the case earlier. Specifically, we considered $19M$ weakly-supervised images (\WS{Image}{Kinetics}{19M}) and $19M$ videos (\WS{Video}{Kinetics}{19M}), whose associated hashtags match the Kinetics label space as our pre-training datasets. The training schedule details are provided in the supplementary material. As discussed earlier (Sec. \ref{sec:vidLengths}), due to temporal jittering, the model considering video frames as input is likely to operate on more number of unique datapoints compared to the model trained on \WS{Image}{Kinetics}{19M} data. To combat this plausible undue advantage to the video input model, we considered another image dataset with $250M$ weakly-supervised images (\WS{Image}{Kinetics}{250M}). The $R3D$ model is pre-trained on an input of $8$-frames per video and a mini-batch size of $16$ videos. \\
\textbf{Key takeaways:} From the results reported in Table \ref{tbl:image2video1}, we may conclude that:
\begin{packed_enum}
\vspace{-0.08in}
\item Pre-training a spatio-temporal model -- $R3D$ -- on video data yields a significant boost of $\boldsymbol{4.28\%}$ ($71.73\%$ vs. $67.45\%$) on Kinetics when compared to the scenario where a spatial model was trained on image / video frames at scale. We may thus conclude that effectively modeling the temporal structure of videos in a very large-scale training setup is extremely beneficial.
\item Despite the structural differences between the image and the video content, pre-training the spatial R2D model on standalone images or random video frames did not make a significant difference in the transfer learning performance. From Table \ref{tbl:image2video1}, we may observe that though R2D model trained on random video frames consistently outperforms other $2D$ inputs, the boost in the performance is marginal (about $\boldsymbol{\sim 0.5\%}$ on average).
\end{packed_enum}
\subsection{Comparisons with state-of-the-art results}\label{sec:sota}
\begin{table}[t]
\footnotesize
\setlength\extrarowheight{1.2pt}
\centering
\begin{center}
\begin{tabular}{|P{2.8cm}|P{1.6cm}|P{0.9cm}|P{1.45cm}|}
\hline
Approach & Pre-training vision data & top-1 acc. & Input type \\
\hhline{|=|=|=|=|}
I3D-Two-Stream \cite{i3d} & ImageNet & 75.7 & RGB + flow \\
\hline
R(2+1)D-Two-Stream~\cite{r2plus1D} & Sports-1M & 75.4 & RGB + flow \\
\hline
3-stream SATT \cite{kinetics17} & ImageNet & 77.7 & RGB + flow + audio \\
\hline
NL I3D \cite{nonlocal} & ImageNet & 77.7 & RGB \\
\hhline{|=|=|=|=|}
R(2+1)D-34 & Sports-1M & 71.72 & RGB \\
\hline
R(2+1)D-34 & \WStwo{Kinetics}{65M} & 79.06 & RGB \\
\hline
Ours (R(2+1)D-152) & \WStwo{Kinetics}{65M} & \textbf{80.49} & RGB
\\
\hline
\end{tabular}
\end{center}
\vspace{-0.1in}
\caption{\footnotesize{Comparison with the state-of-the-art approaches on Kinetics dataset}} \label{tbl:sotaKin}
\vspace{-0.1in}
\end{table}
\begin{table}[t]
\footnotesize
\setlength\extrarowheight{1.2pt}
\centering
\begin{center}
\begin{tabular}{|P{3cm}|P{2.1cm}|P{0.55cm}|P{1cm}|}
\hline
Approach & Pre-training vision data & mAP & Input type \\
\hhline{|=|=|=|=|}
Best number from leader board \cite{epicKitchens1} & -NA- & & -NA- \\
\hhline{|=|=|=|=|}
R(2+1)D-34 \cite{r2plus1D} & Kinetics & & RGB \\
\hline
R(2+1)D-34 \cite{r2plus1D} & Sports-1M & & RGB \\
\hline
R(2+1)D-34 \cite{r2plus1D} & \WStwo{Kinetics}{65M} & & RGB \\
\hline
Ours: R(2+1)D-152 & \WStwo{Kinetics}{65M} & & RGB \\
\hline
\end{tabular}
\end{center}
\vspace{-0.1in}
\caption{\footnotesize{Comparison with the state-of-the-art approaches on Epic-Kitchens dataset}.} \label{tbl:sotaKitchens}
\vspace{-0.1in}
\end{table}
In this section, we compare our best model (R(2+1)D-152, pre-trained on \WStwo{Kinetics}{65M}) with several state-of-the-art approaches on $4$ different target datasets. Unlike all other ablation studies, for the results reported in this section alone, we obtain the final video prediction by processing \textit{each} frame of a test video and compute an average across all frames (as opposed to sampling $10$ uniform clips as mentioned earlier).\note{Add more details on dense sampling + FCN} 

We note that this is not a fair comparison as each approach being compared varies greatly in terms of model architectures, pre-training datasets (ImageNet vs. Sports-1M), amount and type of input data (RGB vs flow vs audio, etc.), input clip size, input frame size, evaluation strategy, and so on. We also note that most prior state-of-the-art models use complex, optimized network architectures compared to ours. Despite these differences, our approach of pre-training R(2+1)D-152 on millions of videos outperforms \underline{all} existing methods by a substantial margin of $\boldsymbol{2.3\%}$ when fully-finetuned on Kinetics (Table \ref{tbl:sotaKin}).

In Table \ref{tbl:sotaKitchens}, we report the performance on the test dataset from the server as part of the Epic-Kitchens Action Recognition Challenge \cite{epicKitchens1}. As baselines, since the training dataset of Epic-Kitchens consists of only $\sim20K$ videos, we pre-train R(2+1)D-34 on Kinetics, Sports-1M, and \WStwo{Kinetics}{65M} separately and fine-tune on Epic-Kitchens test data. We also report the top-performing method from the challenge website at the time of the submission of this manuscript. \note{Compare and report performances.} 

To further illustrate the generalizability of our pre-trained models, we also evaluate on SOA-v1\cite{soa} ($350K$ training and $55K$ test videos), a recently introduced large-scale, multi-label, and multitask video dataset capturing Scenes, Objects, and Actions (SOA) in a given video sequence. As baselines, we train R(2+1)D-34 and 152 layer models from scratch on SOA training data and report the performance in Table \ref{tbl:sotaSOA}. \note{report performance and observations}


% We note that achieving state-of-the-art results on Charades and Something-something requires the development of tailored architectures, e.g., using many image transformations and model ensembles, which is out of the scope of this paper
\begin{table}[t]
\footnotesize
\setlength\extrarowheight{1.2pt}
\centering
\begin{center}
\begin{tabular}{|P{3cm}|P{2.1cm}|P{0.55cm}|P{1cm}|}
\hline
Approach & Pre-training vision data & mAP & Input type \\
\hhline{|=|=|=|=|}
R(2+1)D-34 \cite{r2plus1D} & From scratch & & RGB \\
\hline
Ours: R(2+1)D-34 & \WStwo{Kinetics}{65M} & & RGB \\
\hline
R(2+1)D-152 & From scratch & & RGB \\
\hline
Ours: R(2+1)D-152 & \WStwo{Kinetics}{65M} & & RGB \\
\hline
\end{tabular}
\end{center}
\vspace{-0.1in}
\caption{\footnotesize{Comparison with the state-of-the-art on SOA \cite{soa}.}} \label{tbl:sotaSOA}
\vspace{-0.15in}
\end{table}
\begin{table}[t]
\footnotesize
\setlength\extrarowheight{1.2pt}
\centering
\begin{center}
\begin{tabular}{|P{3cm}|P{2.1cm}|P{0.55cm}|P{1cm}|}
\hline
Approach & Pre-training vision data & mAP & Input type \\
\hhline{|=|=|=|=|}
R(2+1)D-34 \cite{r2plus1D} & Kinetics & & RGB \\
\hline
R(2+1)D-34 \cite{r2plus1D} & Sports-1M & & RGB \\
\hline
R(2+1)D-34 & \WStwo{Kinetics}{65M} & & RGB \\
\hline
R(2+1)D-152 & \WStwo{Kinetics}{65M} & & RGB \\
\hline
Ours: R(2+1)D-152 & \WStwo{Kinetics}{65M} & & RGB \\
\hline
\end{tabular}
\end{center}
\vspace{-0.1in}
\caption{\footnotesize{Comparison with the state-of-the-art on Charades \cite{charades}}} \label{tbl:sotaSOA}
\vspace{-0.15in}
\end{table}

==> relWork_nov13_dhruv.tex <==
\section{Related Work} \label{sec:relatedWork}
\noindent \textbf{Learning from weak supervision: }Given the known challenges in gathering exhaustive annotations for various image and video tasks, leveraging object labels and other meta information to supply weak supervision for object detection and localization\cite{deepDetect, freeLocalization, shi2017transfer, wildcat, visualRelations, paris, weakVideo}, semantic segmentation \cite{segment1, segment2, segment3, segment4, segment5, segment6, segment7}, and other tasks\cite{signLang} are a few widely-adopted strategies. However, we aim to investigate the orthogonal task of transfer of the resulting networks pre-trained on weakly-supervised data to other tasks. Moreover, weak supervision in our approach comes from the lack of temporal localization as well as severe noise in using hashtags for supervision. Although novel changes to the neural architectures have been proposed in the past \cite{noise1, noise2} to combat the noise, we show that large scale training makes the models resilient to noise without doing any structural changes.\\
\noindent\textbf{Dataset sources:} Using Internet as a natural source of content \cite{neil, everything, annotate, im2text, farhadi2010every, bergamo2010exploiting, fergus2010learning, schroff2011harvesting, chen2015webly} and the associated search queries as labels, or hashtags and user-comments from photo-sharing services \cite{f1, f2, f3, uruImage} is a widely-adopted strategy for constructing vision datasets. Most large-scale video datasets \cite{sports1m, youtube8m, yfcc100m} were constructed by first curating a label taxonomy by analyzing the text metadata surrounding YouTube or Flickr videos and some manual cleaning of non-visual labels. \cite{v1, v2, v3, v4} analyzed movie scripts for automatic annotation of human actions to tackle a variety of tasks such as recognizing and localizing actions and actors. Recently there have been increasing efforts to construct synthetic training datasets for a variety of vision tasks \cite{s2,s1,s4,s5,s3,s6,s9,s10,s7,s8}. Our proposed work falls in the first category, i.e., using web-data and the associated text for weak supervision.\\
\noindent \textbf{Pre-training on large datasets:} Since datasets for complex tasks such as object detection, segmentation and action recognition in videos are order of magnitude smaller compared to ImageNet \cite{imagenet}, pre-training on larger, auxiliary data followed by fine-tuning on target tasks \cite{segment, decaf, l2, i3d, r2plus1D, nonlocal, uruImage, jft, laurens} is widely popular. Indeed, a strategy such as \textit{inflation} \cite{i3d} was proposed to exclusively leverage ImageNet instantiation by way of converting $2D$ filters to $3D$, given that training $3D$ models is computationally expensive. In this work, we show that pre-training the models on video clips perform significantly better than pre-training on image/video frames followed by inflation.

==> relatedWork_nov12.tex <==
\section{Related Work} \label{sec:relatedWork}
\noindent \textbf{Learning from weak supervision: }Given the known challenges in gathering exhaustive annotations for various image and video tasks, weakly-supervised pre-training techniques have become increasingly popular. Leveraging object labels \cite{deepDetect, freeLocalization, shi2017transfer, wildcat, visualRelations}, GPS information \cite{paris}, or video data \cite{weakVideo} to supply weak supervision for object detection and localization, semantic segmentation \cite{segment1, segment2, segment3, segment4, segment5, segment6, segment7}, sign language translation \cite{signLang} are a few widely-adopted strategies. Similar to these, our approach also suffers from limited information, since hashtags mostly reflect objects (nouns) and may not provide action-related information contained in the video. \note{How do we defend this statement without being able to share any stats on the data?}. \matt{There are publicly-available lists of top hashtags; we could defer to something like that if we can find a large one} Additionally, our model is also deprived of clean human supervision of labels leading to severe noise. Towards combating this issue, novel structural changes to the neural architectures have been proposed in the past \cite{noise1, noise2}. Contrary to these prior works, we use R(2+1)D \cite{r2plus1D} as our base model without any changes to its architecture and argue that, at very large-scale, models can be trained to be robust to noise.\\
\noindent\textbf{Weakly-supervised datasets: leveraging web, movie scripts, or synthetic data:} Using Internet as a natural source of weakly-supervised content and the associated text to automatically extract labels without explicit manual annotation is a widely-adopted strategy for constructing vision datasets. For instance, using sources such as Google Images \cite{neil, everything, annotate, im2text, farhadi2010every, bergamo2010exploiting, fergus2010learning, schroff2011harvesting, chen2015webly} and the associated search queries as labels, or hashtags and user-comments from photo-sharing services \cite{f1, f2, f3, uruImage} have been very popular. Most large-scale video datasets \cite{sports1m, youtube8m, yfcc100m} were constructed by first curating a label taxonomy by analyzing the text metadata surrounding YouTube or Flickr videos and some manual cleaning of non-visual labels. \cite{v1, v2, v3, v4} analyzed movie scripts for automatic annotation of human actions to tackle a variety of tasks such as recognizing and localizing actions and actors. Recently there have been increasing efforts to construct synthetic training datasets for a variety of vision tasks such as gaze estimation \cite{s2}, font identification \cite{s1}, text localization \cite{s4, s5}, pose estimation \cite{s3,s6, s9, s10}, and semantic segmentation \cite{s7, s8}. Our proposed work falls in the first category, i.e., using web-data and the associated text for weak supervision.\\
\noindent \textbf{Pre-training on large datasets:} Since datasets for complex tasks such as object detection and segmentation are several magnitudes smaller compared to ImageNet \cite{imagenet}, pre-training on larger, auxiliary data followed by fine-tuning on target tasks \cite{segment, decaf, l2, i3d, r2plus1D, nonlocal, uruImage, jft, laurens} is widely popular. Indeed, a strategy such as \textit{inflation} \cite{i3d} was proposed to exclusively leverage ImageNet instantiation by way of converting $2D$ filters to $3D$, given that training $3D$ models is computationally expensive. In this work, we conduct extensive experiments to show the benefit of pre-training clip-based models on large-scale video datasets. We also show in Sec. \ref{sec:image2video} that action recognition significantly benefits from a clip-based model pre-trained on videos compared to $2D$ models pre-trained on image/video frames.

==> relatedWork_old.tex <==
\section{Related Work} \label{sec:relatedWork}
\noindent \textbf{Action recognition datasets:} There are a number of small-scale action recognition datasets such as KTH \cite{kth}, Hollywood-2 \cite{hollywood}, UCF101 \cite{ucf}, Thumos \cite{thumos}, and HMDB \cite{hmdb}, all of which consist of short clips, manually trimmed to capture a single action. Recently, there has been a pivot towards constructing large-scale datasets such as Sports1M \cite{sports1M}, YFCC100M \cite{yfcc100m}, FCVID \cite{fcvid}, Something-something \cite{something-something}, SOA \cite{soa}, Moments in Time \cite{momentsintime}, Kinetics \cite{kinetics}, and so on, all of which consist of a few hundred human action labels ($\sim 600$) and at most a million videos. YouTube-8M \cite{youtube8m}, on the other hand, is the largest public dataset consisting of a total of $6.1M$ videos and $\sim3500$ classes. Though most existing large-scale datasets are constructed on large numbers of untrimmed videos from YouTube, they are well-annotated and also contain temporal localization for each action of interest. Thus, they enable training video models using full supervision. By contrast, our work offers a new way to take advantage of billions of public social media videos and the associated textual metadata such as hashtags to train any video model of choice at scale. \\
\textbf{Video Model Architectures:} All existing video architectures can be categorized into two fundamental categories: (i) frame-based models that utilize $2D$ (spatial only) convolutions and (ii) clip-based models that utilize $3D$ (space-time) convolutions. A systematic comparison of video architectures can be found in \cite{i3d}. 

In frame-based approaches, each video frame is processed independently by utilizing existing top-performing image classification networks to first extract features and then pool them across the input video sequence. A variety of pooling approaches for frame-based models have been proposed in \cite{sports1M, pool1}. A natural extension to such approaches in order to capture temporal information is to add a recurrent layer on top of the last average pooling layer \cite{rnn1, rnn2}. Another class of models construct two-streams-based architectures, where, in addition to RGB, pre-computed optical flow is also considered as input \cite{zisserman, twoStream2}. 

On the other hand, all clip-based models extend the standard $2D$ convolutions to temporal domain resulting in $3D$ filters \cite{3d1, 3d2, 3d3, 3d4, r2plus1D}. These models have a nice property of jointly processing spatial and temporal data thereby effectively capturing low-level spatial and motion variations. However, such models have orders of magnitudes more parameters than $2D$ models and are generally harder to train. To facilitate faster convergence of 3D models, a bootstrapping technique was proposed called \textit{inflation} \cite{i3d} which is now widely-adopted \cite{nonlocal}. The key idea is to convert the pre-trained 2D filters ($N\times N$) to 3D ($N\times N\times k$) by simply repeating the (normalized) $2D$ $N \times N$ weights $k$ times. 

In our work, we chose R(2+1)D as our primary architecture for all our experiments as it jointly captures spatial and temporal information while also incurring lower training costs due to decomposition of the filters \cite{r2plus1D} compared to other $3D$ models.\\
\noindent\textbf{Weakly-supervised large-scale training:} The studies reported in \cite{laurens, jft, uruImage} are the first to thoroughly analyze the effect of very large volumes of pre-training data on various image tasks in a weakly-supervised setting. To the best of our knowledge, this paper is the first to study the effect of million-scale pre-training of video models on feature representations and transfer learning.
\note{Can we write something on pre-training strategies, anything more than i3d}
